Quasi-symmetric functions as polynomial functions on Young diagrams

We determine the most general form of a smooth function on Young diagrams, that is, a polynomial in the interlacing or multirectangular coordinates whose value depends only on the shape of the diagram. We prove that the algebra of such functions is isomorphic to quasi-symmetric functions, and give a noncommutative analog of this result.

==> Russian.tex <==
\begin{figure}[ht]
    \begin{tikzpicture}

      \begin{scope}[draw=black,scale=.5]

          \draw[->,thick] (0,0) -- (6,0);
          \foreach \x in {1, 2, 3, 4, 5}
              { \draw (\x, -2pt) node[anchor=north] {{\tiny{$\x$}}} -- (\x,
2pt); }

          \draw[->,thick] (0,0) -- (0,5);
          \foreach \y in {1, 2, 3, 4}
              { \draw (-2pt,\y) node[anchor=east] {{\tiny{$\y$}}} -- (2pt,\y); }

          \draw[ultra thick,draw=black] (4,0) -- (4,2) -- (2,2) -- (2,3) -- (0,3) ;
          \fill[fill=gray,opacity=0.1] (4,0) -- (4,2) -- (2,2) -- (2,3) -- (0,3) -- (0,0) -- cycle ;
      \end{scope}
 
\begin{scope}[xshift=7cm, yshift=-0cm, scale=0.5]
       \begin{scope}
          \clip (-4.5,0) rectangle (5.5,5.5);
          \draw[thin, dotted] (-6,0) grid (6,6);
          \begin{scope}[rotate=45,draw=gray,scale=sqrt(2)]
              \clip (0,0) rectangle (4.5,5.5);
              \draw[thin, dotted] (0,0) grid (6,6);
          \end{scope}
      \end{scope}

      \draw[->,thick] (-6,0) -- (6,0) node[anchor=west] {\tiny{$x$}};
%      \foreach \z in {-5, -4, -3, -2, -1, 1, 2, 3, 4, 5}
%            { \draw (\z, -2pt) node[anchor=north] {\tiny{$\z$}} -- (\z, 2pt); }

      \draw[->,thick] (0,-0.4) -- (0,6);
%      \foreach \t in {1, 2, 3, 4, 5}
%            { \draw (-2pt,\t) node[anchor=east] {\tiny{$\t$}} -- (2pt,\t); }



% \begin{scope}
%           \clip (5.5,0) rectangle (15.5,5.5);
%           \draw[thin, dotted] (4,0) grid (16,6);
%           \begin{scope}[rotate=45,draw=gray,scale=sqrt(2)]
%               \clip (10,0) rectangle (4.5,5.5);
%               \draw[thin, dotted] (10,0) grid (16,6);
%           \end{scope}
%       \end{scope}
% 
%       \draw[->,thick] (4,0) -- (16,0) node[anchor=west]{$z$};
%       \foreach \z in {5, 6, 7, 8, 9, 11, 12, 13, 14, 15}
%             { \draw (\z, -2pt) node[anchor=north] {\tiny{$\z$}} -- (\z,
% 2pt); }
% 
%       \draw[->,thick] (10,-0.4) -- (10,6) node[anchor=south]{$t$};
%       \foreach \t in {1, 2, 3, 4, 5}
%             { \draw ($(10,0)+(-2pt,\t)$) node[anchor=east] {\tiny{$\t$}} --
% ($(10,0)+(2pt,\t)$); }

     
\begin{scope}[draw=gray,rotate=45,scale=sqrt(2)]

          \draw[->,thick] (0,0) -- (6,0);
%          \foreach \x in {1, 2, 3, 4, 5}
%              { \draw (\x, -2pt) node[anchor=north,rotate=45]
%{\textcolor{gray}{\tiny{$\x$}}} -- (\x, 2pt); }

          \draw[->,thick] (0,0) -- (0,5);
%          \foreach \y in {1, 2, 3, 4}
%              { \draw (-2pt,\y) node[anchor=east,rotate=45]
%{\textcolor{gray}{\tiny{$\y$}}} -- (2pt,\y); }

          \draw[ultra thick,draw=black] (5.5,0) -- (4,0)  -- (4,2) -- (2,2) -- (2,3) --
          (0,3) -- (0,4.5) ;
          \fill[fill=gray,opacity=0.1] (4,0) -- (4,2) -- (2,2) -- (2,3) -- (0,3) -- (0,0) -- cycle ;

      \end{scope}

 \draw[ultra thick,dotted] (4,4) -- (4,0) node[anchor=north] {\tiny{$x_1=4$}};
 \draw[ultra thick,dotted] (2,6) -- (2,-.8) node[anchor=north] {\tiny{$x_2=2$}};
 \draw[ultra thick,dotted] (0,4) -- (0,0) node[anchor=north] {\tiny{$x_3=0$}};
 \draw[ultra thick,dotted] (-1,5) -- (-1,-.8) node[anchor=north] {\tiny{$x_4=-1$}};
 \draw[ultra thick,dotted] (-3,3) -- (-3,0) node[anchor=north] {\tiny{$x_5=-3$}};

\end{scope}

    \end{tikzpicture}


    \caption{Young diagram $\lambda=(4,4,2)$
    and the graph of the associated function $\omega_\lambda$.
%    shown in the French and Russian
%conventions.
%             The solid line represents the profile of the Young diagram.
%             The coordinates system $(z,t)$ corresponding to the
%             Russian convention and the coordinate system $(x,y)$
%             corresponding to the French convention are shown.
}

    \label{FigRussian}
\end{figure}

